WorldReasoner: Evaluating Whether Language Model Agents Forecast Events with Valid Reasoning

Forecasting real-world events requires language-model agents to reason under uncertainty from incomplete, time-bounded information. Yet evaluating whether agents genuinely forecast requires more than final-answer accuracy: a model may be correct by recalling memorized training facts, citing fabricated evidence, or producing an unsupported causal story. We present WorldReasoner, an evaluation framework for temporally valid event forecasting. Each task gives an agent a resolved forecasting question, a simulated forecast date, and access only to evidence available before that date; after resolution, the framework scores the submitted probability, cited evidence, and optional causal event graph. WorldReasoner reports three complementary axes: outcome quality against resolved answers, evidence quality over cited sources, and reasoning quality against post-resolution hindsight graphs. The benchmark is built by an agentic construction pipeline that generates forecasting questions, collects time-stamped evidence, and builds hindsight reference graphs at scale, yielding 345 resolved tasks derived from 14,141 articles with graphs covering 8,087 extracted events. Across six controlled agent settings, temporally valid retrieval is the strongest driver of outcome accuracy; causal graph construction improves key-event recovery; and correct graph-enabled forecasts are more strongly grounded in key events and relevant sources, yet agents still struggle to convert grounded evidence into calibrated probabilities.

==> sections/10_acknowledgments.tex <==
% !TEX root = ../acl_latex.tex
\section*{Acknowledgments}


==> sections/generated/annotation_quality_table.tex <==
% Auto-generated by scripts/analysis/annotation_quality.py
% Generated at 2026-05-22 21:29 UTC
\begin{table*}[tbp]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrrp{0.44\columnwidth}}
\toprule
\textbf{Quality signal} & \textbf{Count} & \textbf{Rate} & \textbf{Interpretation} \\
\midrule
Accepted hindsight events & 336 / 492 & 68.3\% & Events judged real, dated correctly, source-supported, and relevant. \\
Factual-error rejections & 113 / 492 & 23.0\% & Fabricated, wrong-date, or source-mismatch events removed by review. \\
Skipped or unverifiable events & 43 / 492 & 8.7\% & Events left unresolved by annotators rather than forced into a label. \\
\midrule
Source mismatch & 60 / 492 & 12.2\% & Most common factual-error mode. \\
Wrong date & 27 / 492 & 5.5\% & Event occurred, but not at the graph date. \\
Fabricated & 26 / 492 & 5.3\% & Event could not be verified as described. \\
\bottomrule
\end{tabular}
\caption{Annotation-quality summary for the main annotation batch. Annotation review serves as a conservative validation layer for hindsight graphs, while fine-grained event validation remains a nontrivial judgment task.}
\label{tab:annotation_quality}
\end{table*}

